MASSV: Multimodal Adaptation and Self-Data Distillation for Speculative Decoding of Vision-Language Models

Speculative decoding significantly accelerates language model inference by enabling a lightweight draft model to propose multiple tokens that a larger target model verifies simultaneously. However, applying this technique to vision-language models (VLMs) presents two fundamental challenges: small language models that could serve as efficient drafters lack the architectural components to process visual inputs, and their token predictions fail to match those of VLM target models that consider visual context. We introduce Multimodal Adaptation and Self-Data Distillation for Speculative Decoding of Vision-Language Models (MASSV), which transforms existing small language models into effective multimodal drafters through a two-phase approach. MASSV first connects the target VLM's vision encoder to the draft model via a lightweight trainable projector, then applies self-distilled visual instruction tuning using responses generated by the target VLM to align token predictions. Comprehensive experiments across the Qwen2.5-VL and Gemma3 model families demonstrate that MASSV increases accepted length by up to 30% and delivers end-to-end inference speedups of up to 1.46x on visually-grounded tasks. MASSV provides a scalable, architecture-compatible method for accelerating both current and future VLMs.

==> tex_files/results_old.tex <==
\section{Empirical Results}
\label{sec:results}
In this section, we evaluate MASD against text-only drafting with an off-the-shelf LLM. We find that MASD outperforms this baseline across different model families, downstream tasks, and sampling temperatures.

\begin{table*}[!h]
\caption{Mean accepted lengths when drafting across different model families, tasks, and sampling temperatures. "LI 150k" refers to LLaVA Instruct 150 and "COCO" refers to the captioning task on images taken from the COCO Test 2017 dataset.}
\label{sample-table}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lccccccccr}
\toprule
Target Model & Method & LI 150k & LLaVA-Bench & GQA  & COCO & Overall \\
\midrule
\multicolumn{7}{c}{Temperature = 0}\\
\midrule
Qwen2.5-VL 7B Instruct  & Baseline & 2.37                & 2.61                            & 2.59 & 2.21            & 2.46    \\
                       & MASD     & 3.21                & 3.12                            & 3.28 & 3.26            & $\textbf{3.20}_{\textcolor{OliveGreen}{\uparrow0.74}}$   \\
\midrule
Qwen2.5-VL 32B Instruct  & Baseline & 2.46                & 2.70                            & 2.79 & 2.48            & 2.61    \\
& MASD     & 3.12                & 2.90                           & 3.19 & 3.09            & $\textbf{3.04}_{\textcolor{OliveGreen}{\uparrow0.43}}$   \\
\midrule
Gemma 3 12B IT         & Baseline & 2.71                & 2.72                            & 2.75 & 2.84            & 2.76    \\
                       & MASD     & 3.30                 & 3.00                            & 3.07 & 3.41            & $\textbf{3.19}_{\textcolor{OliveGreen}{\uparrow0.43}}$  \\ 
\midrule
Gemma 3 27B IT  & Baseline & 2.49                & 2.70                            & 2.61 & 2.73            & 2.65    \\
& MASD     & 3.00                & 2.84                           & 2.86 & 3.24            & $\textbf{2.99}_{\textcolor{OliveGreen}{\uparrow0.34}}$   \\
\midrule
\multicolumn{7}{c}{Temperature = 1}\\
\midrule
Qwen2.5-VL 7B Instruct & Baseline & 2.47                & 2.75                            & 2.63 & 2.41            & 2.58    \\
                       & MASD     & 3.35                & 2.98                            & 3.19 & 3.31            & $\textbf{3.18}_{\textcolor{OliveGreen}{\uparrow0.60}}$ \\
\midrule
Qwen2.5-VL 32 Instruct  & Baseline & 2.48                & 2.69                            & 2.75 & 2.56            & 2.63    \\
& MASD     & 3.01                & 2.87                           & 3.00 & 3.04            & $\textbf{2.97}_{\textcolor{OliveGreen}{\uparrow0.34}}$   \\
\midrule
Gemma 3 12B IT         & Baseline & 2.67                & 2.79                            & 2.78 & 2.94            & 2.82    \\
                       & MASD     & 3.08                & 2.82                            & 3.01 & 3.37            & $\textbf{3.06}_{\textcolor{OliveGreen}{\uparrow0.24}}$   \\
\midrule
Gemma 3 27B IT  & Baseline & 2.57                & 2.67                            & 2.63 & 2.73            & 2.67    \\
& MASD     & 2.81                & 2.62                           & 2.82 & 3.13            & $\textbf{2.84}_{\textcolor{OliveGreen}{\uparrow0.17}}$   \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\label{mal_table}
\end{table*}

\textbf{Models.} We conduct our experiments with the Qwen2.5-VL Instruct~\citep{bai2025qwen25vltechnicalreport} and instruction-tuned Gemma 3~\citep{gemmateam2025gemma3technicalreport} model families. For Qwen2.5-VL Instruct, we use the 7B model as the target $M_p$ and apply MASD to Qwen2.5-1.5B. For Gemma 3, we use the 12B IT as the target and apply MASD to Gemma3-1B IT. Text-only drafting with the off-the-shelf SLM is our \textit{baseline}.

\textbf{Drafter Training.} We train all draft models on $4\times$ H100s using the following setup and hyperparameters. In the first phase, we pretrain for one epoch on the LLaVA-Pretrain-LCS-558K~\footnote{\url{https://huggingface.co/datasets/liuhaotian/LLaVA-Pretrain}} dataset with a global batch size of 256 and a learning rate of $10^{-3}$. In the second phase, we train for one epoch on the dataset distilled from the LLaVA-mix-665K~\footnote{\url{https://huggingface.co/datasets/liuhaotian/LLaVA-Instruct-150K/blob/main/llava_v1_5_mix665k.json}} dataset using a global batch size of 128 and a learning rate of $2 \times 10^{-5}$. Additional implementation details are provided in the Appendix.

\textbf{Evaluation Tasks.} We evaluate on subsets of 4 datasets: LLaVA Instruct 150k~\citep{liu2023visual}, LLaVA-Bench (In-the-Wild)~\footnote{\url{https://huggingface.co/datasets/liuhaotian/llava-bench-in-the-wild}}, GQA~\citep{Hudson_2019_CVPR}, and image captioning prompts for images from COCO (Test 2017)~\citep{lin2015microsoftcococommonobjects}. The metric used to assess drafting performance is mean accepted length ($\tau$) defined as the expected number of tokens generated per forward call of the target model. It measures the improvement in inference latency independently of the hardware and software implementation used.

\textbf{Inference Settings.} Each drafter is evaluated on $1\times$ H100 using speculation length $\gamma = 5$. We evaluate decoding at temperatures $T \in \{0, 1\}$.

\textbf{Results.} As shown in Figure \ref{fig:qwen_mal}, MASD achieves higher mean accepted lengths than the baseline and MASD w/o SDD for the Qwen2.5-VL 7B Instruct target across all tasks when drafting at temperature $T = 0$. Note that the poorest performance of the text-only baseline and the greatest improvement yielded by the MASD drafter (47.5\%) are both on the COCO Captioning category. This highlights the need for a multimodal drafter when the target VLM is performing tasks such as image captioning, where the outputs are almost entirely determined by visual information.

Table \ref{mal_table} shows that our method is also effective for adapting Gemma 3 1B IT into a VLM drafter for Gemma 3 12B IT, despite the architectures of the Qwen2.5-VL and Gemma 3 model families differing substantially (i.e., Qwen2.5-VL models use a dynamic number of visual tokens; Gemma 3 models use interleaved sliding window attention). These findings validate that MASD produces drafters aligned to the target model's multimodal distribution, while being able to handle different model architectures and downstream tasks.

% \section{Empirical Results}
% \label{sec:results}
% In this section, we evaluate MASD against text-only drafting with an off-the-shelf LLM. We find that MASD outperforms this baseline across different model families, downstream tasks, and sampling temperatures.

% \begin{table*}[!h]
% \caption{Mean accepted lengths when drafting across different model families, tasks, and sampling temperatures. "LI 150k" refers to LLaVA Instruct 150 and "COCO" refers to the captioning task on images taken from the COCO Test 2017 dataset.}
% \label{sample-table}
% \vskip 0.15in
% \begin{center}
% \begin{small}
% \begin{sc}
% \begin{tabular}{lccccccccr}
% \toprule
% Target Model & Method & LI 150k & LLaVA-Bench & GQA  & COCO & Overall \\
% \midrule
% \multicolumn{7}{c}{Temperature = 0}\\
% \midrule
% Qwen2.5-VL 7B Instruct  & Baseline & 2.37                & 2.61                            & 2.59 & 2.21            & 2.46    \\
%                        & MASD     & 3.21                & 3.12                            & 3.28 & 3.26            & $\textbf{3.20}_{\textcolor{OliveGreen}{\uparrow0.74}}$   \\
% \midrule
% Qwen2.5-VL 32B Instruct  & Baseline & 2.46                & 2.70                            & 2.79 & 2.48            & 2.61    \\
% & MASD     & 3.12                & 2.90                           & 3.19 & 3.09            & $\textbf{3.04}_{\textcolor{OliveGreen}{\uparrow0.43}}$   \\
% \midrule
% Gemma 3 12B IT         & Baseline & 2.71                & 2.72                            & 2.75 & 2.84            & 2.76    \\
%                        & MASD     & 3.30                 & 3.00                            & 3.07 & 3.41            & $\textbf{3.19}_{\textcolor{OliveGreen}{\uparrow0.43}}$  \\ 
% \midrule
% Gemma 3 27B IT  & Baseline & 2.49                & 2.70                            & 2.61 & 2.73            & 2.65    \\
% & MASD     & 3.00                & 2.84                           & 2.86 & 3.24            & $\textbf{2.99}_{\textcolor{OliveGreen}{\uparrow0.34}}$   \\
% \midrule
% \multicolumn{7}{c}{Temperature = 1}\\
% \midrule
% Qwen2.5-VL 7B Instruct & Baseline & 2.47                & 2.75                            & 2.63 & 2.41            & 2.58    \\
%                        & MASD     & 3.35                & 2.98                            & 3.19 & 3.31            & $\textbf{3.18}_{\textcolor{OliveGreen}{\uparrow0.60}}$ \\
% \midrule
% Qwen2.5-VL 32 Instruct  & Baseline & 2.48                & 2.69                            & 2.75 & 2.56            & 2.63    \\
% & MASD     & 3.01                & 2.87                           & 3.00 & 3.04            & $\textbf{2.97}_{\textcolor{OliveGreen}{\uparrow0.34}}$   \\
% \midrule
% Gemma 3 12B IT         & Baseline & 2.67                & 2.79                            & 2.78 & 2.94            & 2.82    \\
%                        & MASD     & 3.08                & 2.82                            & 3.01 & 3.37            & $\textbf{3.06}_{\textcolor{OliveGreen}{\uparrow0.24}}$   \\
% \midrule
% Gemma 3 27B IT  & Baseline & 2.57                & 2.67                            & 2.63 & 2.73            & 2.67    \\
% & MASD     & 2.81                & 2.62                           & 2.82 & 3.13            & $\textbf{2.84}_{\textcolor{OliveGreen}{\uparrow0.17}}$   \\
% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% \vskip -0.1in
% \label{mal_table}
% \end{table*}

% \textbf{Models.} We conduct our experiments with the Qwen2.5-VL Instruct~\citep{bai2025qwen25vltechnicalreport} and instruction-tuned Gemma 3~\citep{gemmateam2025gemma3technicalreport} model families. For Qwen2.5-VL Instruct, we use the 7B as the target and apply MASD to Qwen2.5 1.5B. For Gemma 3, we use the 12B as the target and apply MASD to the 1B. Text-only drafting with the off-the-shelf LLM is our baseline.

% \textbf{Drafter Training.} We train all draft models on $4\times$ H100s using the following hyperparameters. In the first phase, we pretrain for one epoch on the "LLaVA Visual Instruct Pretrain LCS-558K" dataset with a global batch size of 256 and a learning rate of 1e-3. In the second phase, we train for one epoch on the dataset distilled from the "LLaVA mix665k" dataset using a global batch size of 128 and a learning rate of 2e-5. More details provided in the Appendix.

% \textbf{Evaluation Task.} We evaluate on subsets of 4 datasets: LLaVA Instruct 150k, LLaVA-Bench (In-the-Wild), GQA, and image captioning prompts for images from COCO (Test 2017). The metric used to assess drafting performance is mean accepted length ($\tau$): the expected number of tokens generated per forward call of the target model. It measures the improvement in inference latency independently of the hardware and software implementation used.


% \textbf{Inference Settings.} Each drafter is evaluated on $1\times$ H100 using speculation length 5. We evaluate decoding at temperatures = 0 and 1. 

% \textbf{Results.} As shown in Figure \ref{fig:qwen_mal}, MASD achieves higher mean accepted lengths than the baseline and MASD w/o SDD for the Qwen2.5-VL 7B Instruct target across all tasks when drafting at temperature = 0. Note that the poorest performance of the text-only baseline and the greatest improvement yielded by the MASD drafter (47.5\%) are both on the COCO Captioning category. This highlights the need for a multimodal drafter when the target VLM is performing tasks such as image captioning, where the outputs are almost entirely determined by visual information.

% Table \ref{mal_table} shows that our method is also effective for adapting Gemma 3 1B IT into a VLM drafter for Gemma 3 12B IT, despite the architectures of the Qwen2.5-VL and Gemma 3 model families differing substantially (i.e. Qwen2.5-VL models use a dynamic number of visual tokens; Gemma 3 models use interleaved sliding window attention). These findings validate that MASD produces drafters aligned to the target model's multimodal distribution, while being able to handle different model architectures and downstream tasks.
